CheckINN: Wide Range Neural Network Verification in Imandra (Extended)

Neural networks are increasingly relied upon as components of complex safety-critical systems such as autonomous vehicles. There is high demand for tools and methods that embed neural network verification in a larger verification cycle. However, neural network verification is difficult due to a wide range of verification properties of interest, each typically only amenable to verification in specialised solvers. In this paper, we show how Imandra, a functional programming language and a theorem prover originally designed for verification, validation and simulation of financial infrastructure can offer a holistic infrastructure for neural network verification. We develop a novel library CheckINN that formalises neural networks in Imandra, and covers different important facets of neural network verification.

==> Appendices/1_ACAS_Xu_results.tex <==
\section{Results on Pruned ACAS Xu Benchmark}\label{ap:acas}

Fig.~\ref{fig:acas} shows some indicative experiments running \checkinn on the properties and networks from the ACAS Xu benchmark~\cite{katz_reluplex_2017}. Note that the networks were pruned at 90\% of their weights using static pruning by weight magnitude. The verification was ran on virtual machines with four 2.6 GHz Intel Ice Lake virtual processors and 16GB RAM. Timeout was set at 5 minutes. 

\begin{figure*}
	\caption{Results of experiments ran on the properties and networks from the ACAS Xu benchmark~\cite{katz_reluplex_2017}. The verifications were run on virtual machines with four 2.6 GHz Intel Ice Lake virtual processors and 16GB RAM. Timeout was set at 5 hours}\label{fig:acas}
	\centering
	\begin{tabular}{{ P{1.2cm} P{1.7cm} P{1.7cm} P{1.3cm} P{1.7cm} P{1.3cm} P{1.7cm} P{1.3cm} }}
		\toprule
		
		\multicolumn{2}{P{3.3cm}}{} &
		\multicolumn{2}{P{3.1cm}}{\textbf{CheckINN: Pruned and Quantised Networks}} &
		\multicolumn{2}{P{3.1cm}}{\textbf{CheckINN: Pruned Networks}} &
		\multicolumn{2}{P{3.6cm}}{\textbf{Reluplex: Full ACAS Xu Networks}} \\

		\cmidrule(rl){3-4} \cmidrule(rl){5-6} \cmidrule(rl){7-8}
		
		\textbf{Property} & \textbf{Result} & Quantity & Time (s) & Quantity & Time (s) & Quantity & Time (s) \\ 

		% Property 1
		\rowcolor{lavender}
		$\phi1$ & SAT 		& 4  & 258	& 20 & 13387 	& 0  &			\\
		\rowcolor{lavender}
				& UNSAT 	& 0  & 		& 0	 & 		 	& 41 & 394517	\\
		\rowcolor{lavender}
				& TIMEOUT 	& 5  & 		& 24 & 			& 4  &			\\

		% Property 2
		$\phi2$ & SAT 		&    & 		& 7  & 2098 	& 35 & 82419	\\
				& UNSAT 	& 0  & 		& 2	 & 896	 	& 1  & 463		\\
				& TIMEOUT 	&    & 		& 26 & 			& 4  &			\\

		% Property 3
		\rowcolor{lavender}
		$\phi3$ & SAT 		&    & 		& 39 & 10453 	& 35 & 82419	\\
		\rowcolor{lavender}
				& UNSAT 	& 0  & 		& 0	 & 		 	& 1  & 463		\\
		\rowcolor{lavender}
				& TIMEOUT 	&    & 		& 2  & 			& 4  &			\\

		% Property 4
		$\phi4$ & SAT 		& 16 & 1422	& 36 & 21533	& 0  & 		 	\\
				& UNSAT 	& 1  & 114	& 0  & 			& 32 & 12475 	\\
				& TIMEOUT 	& 18 & 3	& 5  & 			& 0  &			\\

		% Property 5
		\rowcolor{lavender}
		$\phi5$ & SAT 		& 1  & 57	& 1  & 98	 	& 0  & 			\\
		\rowcolor{lavender}
				& UNSAT 	& 0  &		& 0  & 		 	& 1	 & 19355	\\

		% Property 6
		$\phi6$ & SAT 		& 1  & 196  & 1  & 98		& 0  &			\\
				& UNSAT 	& 0  & 		& 0  & 			& 1  & 180288	\\

		% Property 7
		\rowcolor{lavender}
		$\phi7$ & TIMEOUT 	& 1	 &		& 1  &	 		& 1  & 			\\

		% Property 8
		$\phi8$ & SAT 		& 0  & 		& 0  & 			& 1  & 40102 	\\
				& TIMEOUT 	& 1  & 		& 1  & 			& 0  & 			\\

		% Property 9
		\rowcolor{lavender}
		$\phi9$ & SAT		& 1  & 66	& 1  & 109	 	& 0  & 			\\
		\rowcolor{lavender}
				& UNSAT		& 0  &		& 0  & 			& 1  & 99634 	\\

		% Property 10
		$\phi10$ & SAT		& 1 & 116	& 0  &			& 0  &			\\
				 & UNSAT 	& 0 & 		& 1  & 637 		& 1  & 19944	\\
				 & TIMEOUT 	& 0 & 		& 0  &	 		& 0 &			\\
		\bottomrule
	\end{tabular}
\end{figure*}	

%property,result,network,time
%6,proved,1,195.633395
%8,timeout,1,0.0
%9,proved,1,66.187463
%10,proved,1,116.369745

==> Appendices/2_extreme_values_lemma_proofs.tex <==
\section{Extreme Values Lemma's Proof}

In this section we provide proofs for the Extreme Values Lemma presented in the main text~\ref{lem:extreme} in the two specific cases \emph{R1} and \emph{R2}. We re-use the same notation as in the lemma's definition(cf. Section~\ref{subsec:structural_property}).

\begin{lemma}[Extreme Values]
	Let $a$ be a vector $a_1, \ldots , a_n$ with distinct pattern and extreme values $a_1, \ldots , a_m$. If for  $w^x$ and $w^y$, we have 
	\begin{equation}\label{eq:extr_val0}
	w^x_1 > w^y_1 \land \ldots \land w^x_m > w^y_m,
	\end{equation}
	
	then 
	\begin{equation}\label{eq:extr_val1}
	(a_1  w^x_1 + \ldots + a_n  w^x_n) > (a_1  w^y_1 + \ldots + a_n w^y_n) .
	\end{equation}
	
\end{lemma} 

\subsection{Case 1: Binary Pooling Layer Output}
Condition \textbf{R1}: $a$ is a binary vector, and $a_{min} \neq a^*, a_{max} \neq a^*$ 

For $a_1, ..., a_m \in a_{ex}$ we need to have 
$$a_1 =\ldots = a_m = 1$$
as
$a^* \neq a_{max} \neq a_{min}$

For $a_{m+1}, \ldots, a_n$ we need to have 
$$a_{m+1} = \ldots = a_n = 0$$ 
as $a^* \neq a_{max} \neq a_{min}$.

Then we have 
$$w_1^x + \ldots + w_m^y > w_1^y + \ldots + w_m^y$$
as (\ref{eq:extr_val1}). This holds because by (\ref{eq:extr_val0}), 
$w_i^x > w_i^y$ for $i \in [1,m]$.


\subsection{Case 2: Binary Pooling Layer Output}

Condition \textbf{R2}: $w_x$ and $w_y$ are binary vectors, $a^* \neq 0$

We suppose that $a_1, \ldots, a_m$ are the smallest possible, i.e. close to $a^* + \frac{a_{max} - a^*}{2}$
and $a_{m+1}, \ldots, a_n$ are the greatest possible, i.e. close to $a^*$

since $w^x$ and $w^y$ are binary, and $w_1^x > w_1^y, \ldots, w_m^x > w_m^y$, we know that 
$$ w_1^x = \ldots = w_m^x = 1$$
$$ w_1^y = \ldots = w_m^y = 0$$

We need to prove that
\begin{align*}
m \left(a^* + \frac{a_{max} - a^*}{2}\right) &> (n-m)a^* \\
1.5 m a^* + \frac{m a_{max}}{2} &> na^* \\
1.5 m + \frac{m a_{max}}{2a^*} &> n \\
m\left(1.5 +\frac{a_{max}}{2a^*}\right) &> n
\end{align*}


We know that $m < n$, so the condition is $m$ has to be \emph{at least} $\frac{n}{1.5 + \frac{a_{max}}{2a^*}}$


==> Sections/7_Explainability.tex <==

\section{Explainability and Neural Network Simulation}\label{sec:explain}
\knote{Explain the point of using Imandra for this}
Finally, we show-case the feature of Imandra that is perhaps
under-valued in the ITP community but proves very important and useful in practice
-- \emph{simulation}, or a facility for running the code within the proof
environment. Because Imandra code is also efficiently executable OCaml code,
we do not need to perform any code extraction to run functions; formal models
are executable ``out of the box.''

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/filter_intuition.png}
	%	\rule{35em}{0.5pt}
	\caption[Filters property intuition]{\footnotesize{\emph{A $2 \times 2$ filter matched with happy images.}}}
	\label{fig:filter_intuition}
\end{figure}
Explaining properties of neural networks has become an active research topic,
within a broad initiative of \emph{explainable
	AI}~\cite{Ribeiro0G16,LundbergL17}. An iconic application of the idea is a task
of detecting forms of bias or unfairness in neural network's decision. This
problem has been explored by the formal logic community e.g.\
in~\cite{UrbanCWZ20,MazzucatoU21}. But, unlike applications that process nominal
data, computer vision data can hardly rely on analysis of individual pixels. The
design of CNNs tries to partially address this problem, as CNN filters are
designed to learn more abstract features in data. We thus conjecture that,
instead of reasoning at the level of individual pixels, our analysis of CNNs can
rely on detecting e.g.\ vertical, horizontal and diagonal lines in the filters.
In this section we return to the CNN library introduced in Section~\ref{sec:CNN}
and experiment with Imandra's capacity to support this kind of analysis.



To make the above intuition more concrete, let us return to the running example
of the data set with happy faces. Looking at the data, it would not be difficult
for a human observer to conclude that a happy face is one that smiles, and a
smile usually (partially) manifests itself as an upper left diagonal in the
mouth region.


A set of CNN filters that would agree with this explanation of a smile should give rise to \emph{heatmaps} that show diagonal lines, as in the top row of Fig.~\ref{fig:diagonal_filters}.
Recall that filters are real matrices;  heatmaps are visualisations of such matrices, where intensity of colours corresponds to values of matrix elements.
In particular,  in Fig.~\ref{fig:diagonal_filters}, black stands for $0$ and white for $1$. 


\begin{figure}
	\centering
	\includegraphics[width=0.2\textwidth]{Figures/exp_filters_diagonal.png}
	\includegraphics[width=0.2\textwidth]{Figures/exp_filters.png}
	%	\rule{35em}{0.5pt}
	\caption[Imposed filters visualisation]{\footnotesize{\emph{Heatmaps of $2\times2\times1$ filters. Top: human-imposed; Bottom: learnt by CNN}}}
	\label{fig:diagonal_filters}
\end{figure}
However, when we train a 100\% accurate CNN and examine heatmaps of the filters it learnt, we notice that in fact it learnt the filters shown at the bottom of Fig.~\ref{fig:diagonal_filters}.
It is not immediately clear how to interpret what the CNN thinks a smile is; and whether we should trust decisions made by the CNN when it encounters yet unseen examples?
Imandra can provide some lightweight support for analysis of such cases.


First of all, having the Imandra formalisation of CNNs, we can simply replace learnt filters with the ones we find intuitive, and, after re-training some other weights of the CNN, we can execute the CNN with ``correct filters'' and confirm that our proposed filter gives 100\% accuracy performance as well, see~\cite{DPKD22}.
In cases when we do not have prior assumptions what the filters should be, we can use Imandra to formalise and test our conjectures about the shapes of filters as given.  

For example, Fig.~\ref{fig:filter_intuition} shows how the first filter in the bottom row of Fig.~\ref{fig:diagonal_filters} matches pictures from the dataset. 
It seems the network learnt to identify corners in images!
To express this conjecture, we implement functions that check patterns in 2$\times$2 matrices.  % (see Listing~\ref{lst:filter_properties}):
For example, ``top right corner''  is shown on the bottom-left filter of Fig.~\ref{fig:diagonal_filters}:

%caption=Example of filter pattern definition in Imandra,
\begin{lstlisting}[label={lst:filter_properties},  language=caml]
	let is_topright_corner m = 
	let is_valid = Matrix.dimensions m =  (2, 2) in
	let tl = Matrix.nth (0, 0) m in
	let tr = Matrix.nth (0, 1) m in
	let bl = Matrix.nth (1, 0) m in
	let br = Matrix.nth (1, 1) m in
	if is_valid && (bl <? tr) &&? (tl <? tr) &&? (br <? tr) = (Ok true)
	then (Ok true) else (Ok false)
\end{lstlisting}

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{Figures/designing_properties.png}
	%	\rule{35em}{0.5pt}
	\caption[Designing pooling layer properties]{\emph{\footnotesize{Pattern propagation through layers}}}
	\label{fig:properties_design}
\end{figure}
\noindent
Our library's matrix implementation helps us formalise these properties easily. We only need to define %useful functions: \lstinline{is_approx}, which compares the equality of two values within a given precision, and
comparison operators for \lstinline{Result} type (\lstinline{<?, ||?, &&?}).



Now we can check in Imandra whether this pattern matches the mouth area's left side for all happy images in the data set, but this does not hold, which means the shape of the filter alone does not explain the 100\% accuracy of the CNN.  
We then conjecture that this filter produces specific patterns in the feature map, which in turn results in specific patterns in the pooling layer, as Fig.~\ref{fig:properties_design}
shows. 


By considering different patterns in the pooling layer, we can express a property
that provides an explanation to the CNN accuracy, i.e.\ it applies to the pooling layer for all happy inputs: the bottom left part of the pooling layer
has a ``top right corner'' pattern -- a property that is not very natural and is defined disjunctively below (\lstinline{tl}) and (\lstinline{bl}) stand for ``top left'' and ``bottom right'' patterns respectively:
\knote{this was not clear in ITP, explain better}
% We implement it using the pattern functions from the previous Listing:
% (* filter presents a negative top - right corner pattern *)
\begin{lstlisting}[label={lst:p1}, language=caml]
	let happy_properties (l: (real Matrix.matrix list)) = 
	...
	let bl_angle = filter >>= is_bottomleft_angle in
	left_vertical ||? bottom_horizontal ||? left_diagonal
	||? tl_corner ||? bl_angle
\end{lstlisting}
%where \lstinline{left_vertical}, \lstinline{bottom_horizontal} etc. are various shapes that we define in the library.

At this stage, we may decide that the learnt property that we iteratively
discovered with Imandra's help is too riddled to provide a sensible explanation,
and we can come up with a better alternative explanation of a smile.
For example, using our diagonal filters as in Fig.~\ref{fig:diagonal_filters}
gives very intuitive geometric explanation, without sacrificing accuracy.
The capacity to simulate neural networks within the prover gives us a
lightweight way to conjecture or impose assumptions on the object of study, and
this capacity can be useful on its own, as well as a way of exploring
potentially interesting verification properties. % in a larger verificationproject.
%(see Figure~\ref{fig:filter_intuition}). It is more interesting to reason about the pooling layer, as it is smaller and only keeps the feature map's most significant values.


